Detoxifying Text with MaRCo: Controllable Revision with Experts and Anti-Experts

Text detoxification has the potential to mitigate the harms of toxicity by rephrasing text to remove offensive meaning, but subtle toxicity remains challenging to tackle. We introduce MaRCo, a detoxification algorithm that combines controllable generation and text rewriting methods using a Product of Experts with autoencoder language models (LMs). MaRCo uses likelihoods under a non-toxic LM (expert) and a toxic LM (anti-expert) to find candidate words to mask and potentially replace. We evaluate our method on several subtle toxicity and microaggressions datasets, and show that it not only outperforms baselines on automatic metrics, but MaRCo's rewrites are preferred 2.1 $\times$ more in human evaluation. Its applicability to instances of subtle toxicity is especially promising, demonstrating a path forward for addressing increasingly elusive online hate.

==> sections/05-related-work.tex <==
\section{Related Work}
% \maarten{I high-key don't think we need this section tbh... As long as we cite all the right papers in section 2, we should be good.}
Some prior detoxification efforts have mild success by replacing a list of swearwords/other explicit toxicity signals \cite{tran-etal-2020-towards, dale-etal-2021-text}.  However, these approaches are weaker on subtly toxic sentences, since these signals are not as apparent in texts such as microagressions. Other work has tried sequence-to-sequence methods where generated tokens are chosen to maximize the likelihood that the sequence is not toxic \cite{dale-etal-2021-text, nogueira-dos-santos-etal-2018-fighting}.
%Contrary to \methodname, ParaGedi uses two LMs.

Adjacent to detoxification,  \citet{ma-etal-2020-powertransformer} use rewriting to give more agency and power to groups in texts with undesirable biases, while 

% \maarten{for the new version, maybe focus on the other rewriting methods for detoxification, and maybe add a paragraph on other stylistic rewriting tasks (e.g., sentiment, PowerTransformer, formality, etc).}


% \begin{itemize}
%     \item \citeauthor{he-etal-2021-detect-perturb} introduce a ``Detect and Preturb'' framework for style transfer, where they first detect sensitive tokens in the original text, then replace them in decoding time.
    
%     Our proposed method differs in that we identify \emph{potentially} sensitive tokens, and \emph{optionally} replace them. Due to the harms of toxic content, it is better to be less sensitive \sh{Can't think of the word I'm looking for! something that means we can be more broadly encompassing} when choosing which tokens to mask. Even if the initial model is overambitious in identifying potentially sensitive tokens, the controlled generation step will retain non-toxic content. If the threshold for sensitive tokens is too small, more subtle, implicit toxicity may persist. 
    
    
%     \item \citealp{malmi-etal-2020-unsupervised} use two, padded masking language models $M_1$ and $M_2$, finetuned on $S_1$ and $S_2$ respectively, and iterate over all subspans of the original text $t$ to identify spans to mask. Next, they fill in these masked spans with predicted tokens from $M_2$. There are a few drawbacks to this approach. First, it is computationally expensive. If $t$ has length $n$, then it takes $\mathcal{O}(n^2)$ model calls to evaluate the spans to mask. In addition, each masked span is replaced with no reference to the original text before masking, so a rewrite $t'$ can easily differ in meaning from $t$ if it maximizes the differences between $M_1$ and $M_2$.
% \end{itemize}

==> sections/09-acknowledgements.tex <==
\section*{Acknowledgements}
We thank Gary Liu, the MTurkers, 

==> tables/bbf.tex <==
\begin{table*}[t]
\footnotesize
\centering
\begin{tabular}{lllllllllll}
\toprule
          & \multicolumn{6}{c}{Validation}         & \multicolumn{4}{c}{Test}               \\
          \cmidrule(lr){2-7}  \cmidrule(lr){8-11}
          & Toxicity & BERTScore & BLEU4 & Fluency & Cnd. Fluency & Cnd. BERTScore & Toxicity & BERTScore& BLEU4  & Fluency \\ \midrule 
Original &   0.177	& --	 & 	-- &	565.116	       & 381.943      & --         \\
CondBERT &   0.123	&	0.974 & 0.867	& 440.982   &        287.227 &	0.989   &           &         \\
CondBERT (ctx) &   0.149	&	0.986 &	0.927	& 473.261&	284.293 &	0.994  &           &         \\

ParaGeDi &   0.099	&	0.940 &	0.621&		252.794&	158.098	&	0.973 \\
ParaGeDi (ctx) &   0.099& 0.939	&0.598	&230.903	&129.500&	0.974 \\
\methodname   &   0.073	&	0.940&	0.688&	230.960	&153.921&	0.977     \\
\methodname (ctx)  & 0.090	&	0.945	& 0.701 &	318.400	& 192.683	& 0.979    \\
\bottomrule
\end{tabular}
\caption{Automatic evaluations on detoxified generations on the BBF dataset for \methodname, ParaGeDi and CondBERT. \methodname achieves the lowest toxicity and best fluency with and wtihout context, and the second-best meaning preservation metrics. Adding context has mixed results, but increases the conditional fluency and BERTScore in CondBERT and ParaGeDi.  }
\label{tab:bbf_auto}
\end{table*}


\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{images/bbf_condbert_marco.png}
        \includegraphics[width=0.5\textwidth]{images/bbf_paragedi_marco.png}
    \caption{Automatic evaluations on detoxified generations on the BBF dataset for \methodname vs ParaGeDi and \methodname vs CondBERT. \methodname is less toxic and less fluent than both baselines. It has better meaning preservation over CondBERT and marginally worse for ParaGeDi}
    \label{fig:bbf_human}
\end{figure}


==> tables/context.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{images/bbf_context.png}
    \caption{Human evaluations on detoxified generations on the BBF dataset for \methodname, ParaGeDi, and CondBERT, with and without context. Utilizing context lead to large gains in reduced toxicity and topicality for ParaGeDi, and moderate gains in these for \methodname. For CondBERT, utilzing context lead to slightly more toxic generations, although the difference was small. For all, including context hardly affected fluency.}
    \label{fig:bbf_context}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{images/ds_context.png}
    \caption{Human evaluations on detoxified generations on the diasafety dataset for \methodname, ParaGeDi, and CondBERT, with and without context. Utilizing context lead to reductions in toxicity, but also in fluency and topicality for ParaGedi. For \methodname, including context lead to slight gains in topicality and reduced toxicity with decreases in fluency. Finally, for CondBERT, utilzing context lead to more toxic and less topical generations with slightly higher fluency.\sh{This is maybe because condbert doesn't change much with or without context- overwhelming metric is ``tie''. plus, it is getting most similar embedding to original word that it's replacing, so if we add a toxic context, it's more likely to retreive a negative word}}
    \label{fig:ds_context}
\end{figure}

==> tables/diasafety.tex <==
\begin{table*}[t]
\footnotesize
\centering
\begin{tabular}{lllllllllll}
\toprule
          & \multicolumn{6}{c}{Validation}         & \multicolumn{4}{c}{Test}               \\
          \cmidrule(lr){2-7}  \cmidrule(lr){8-11}
          & Toxicity & BERTScore & BLEU4 & Fluency & Cnd. Fluency & Cnd. BERTScore & Toxicity & BERTScore& BLEU4  & Fluency \\ \midrule 
Original &   0.262 &--	& --	 & 	-- &341.855        & --         \\
CondBERT &  0.140	&	0.966&	0.837&	259.527&	231.015  &       0.981    &         \\
CondBERT (ctx) &  0.197&	0.977&	0.897&	335.051	&439.979&	0.989  &           &         \\

ParaGeDi &   0.119&	0.924&	0.514&	238.249	&114.234&	0.970\\
ParaGeDi (ctx) & 0.104	&	0.892&	0.286&	317.487&	268.995	&0.961 \\
\methodname   &  0.118&	0.948&	0.736&	168.240&	106.577	&0.979    \\
\methodname (ctx)  & 0.130&		0.939&	0.686&	156.930	&76.029&	0.977    \\
\bottomrule
\end{tabular}
\caption{Automatic evaluations on detoxified generations on the diasafety dataset for \methodname, ParaGeDi and CondBERT. ParaGeDi context achieves the lowest toxicity overall, CondBERT has the best meaning preservation, and \methodname has the best fluency. Adding context has mixed results - in some cases, it decreases fluency and toxicity, while in some cases it increases it}
\label{tab:ds_auto}
\end{table*}

\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{images/ds_condbert_marco.png}
        \includegraphics[width=0.5\textwidth]{images/ds_paragedi_marco.png}
    \caption{Automatic evaluations on detoxified generations on the Diasafety dataset for \methodname vs ParaGeDi and \methodname vs CondBERT. Compared to CondBERT, \methodname is less toxic, marginally better at preserving meaning, and marginally less fluent. Compared to ParaGeDi, \methodname has worse meaning preservation and toxicity, but is slighlty more fluent.}
    \label{fig:ds_human}
\end{figure}


==> tables/dynabench.tex <==
\begin{table}[t]
\footnotesize
\centering
\begin{tabular}{lllll}
\toprule
          & \multicolumn{4}{c}{Validation}            \\
          \cmidrule(lr){2-5}  
          & Toxicity & BERTScore & BLEU4 & Fluency \\ \midrule
Original &   0.563	& --	 & 	-- &	426.07      \\
CondBERT &   \underline{0.288}	&	\textbf{0.954} & \textbf{0.784}	& \underline{259.33}       \\
ParaGeDi  &     0.332 &	 0.918 &	0.501 &385.15        \\
MaRCo     &     \textbf{0.274}	&	\underline{0.939}	& \underline{0.706} &	\textbf{146.01}         \\ \bottomrule
\end{tabular}
\caption{Automatic evaluations on detoxified generations on the DynaHate dataset for \methodname, ParaGeDi and CondBERT. \methodname achieves the lowest toxicity and best fluency, and the second-best meaning preservation metrics. CondBERT achieves the highest BERTScore and BLEU4.  }
\label{tab:3}
\end{table}
% \begin{table*}[t]
% \footnotesize
% \centering
% \begin{tabular}{lllllllll}
% \toprule
%           & \multicolumn{4}{c}{Validation}         & \multicolumn{4}{c}{Test}               \\
%           \cmidrule(lr){2-5}  \cmidrule(lr){6-9}
%           & Toxicity & BERTScore & BLEU4 & Fluency & Toxicity & BERTScore& BLEU4  & Fluency \\ \midrule
% Original &   0.563	& --	 & 	-- &	426.07             &       &         \\
% CondBERT &   \underline{0.288}	&	\textbf{0.954} & \textbf{0.784}	& \underline{259.33}              &           &         \\
% ParaGeDi  &     0.332 &	 0.918 &	0.501 &385.15  &           &        \\
% MaRCo     &     \textbf{0.274}	&	\underline{0.939}	& \underline{0.706} &	\textbf{146.01}         &           &       \\ \bottomrule
% \end{tabular}
% \caption{Automatic evaluations on detoxified generations on the DynaHate dataset for \methodname, ParaGeDi and CondBERT. \methodname achieves the lowest toxicity and best fluency, and the second-best meaning preservation metrics. CondBERT achieves the highest BERTScore and BLEU4.  }
% \label{tab:3}
% \end{table*}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\textwidth]{images/dynabench_paragedi_marco.png}
%         \includegraphics[width=0.5\textwidth]{images/dynabench_condbert_marco.png}
%     \caption{Human evaluations on detoxified generations on the DynaHate dataset for \methodname vs ParaGeDi and for \methodname vs CondBERT. \methodname has less-toxic and more fluent generations, while both CondBERT and ParaGeDi has more meaning preservation.}
%     \label{fig:dynabench_marco_paragedi}
% \end{figure}

==> tables/microagressions.tex <==
\begin{table}[t]
\footnotesize
\centering
\begin{tabular}{@{}lrrrr@{}}
\toprule
          & \multicolumn{4}{c}{Validation}           \\
          \cmidrule(lr){2-5} 
          & Toxicity & BERTScore & BLEU4 & PPL
          \\ \midrule
Original & 0.286  & --	 & 	-- &         80.54         \\
CondBERT &   \underline{0.161}	& \textbf{0.966} &	\textbf{0.800} &	\underline{114.27}                      \\
ParaGeDi  &     0.162	& 0.931 &	0.499 &	140.86               \\
MaRCo     &      \textbf{0.145} & \underline{0.958} &	\underline{0.768} &	\textbf{61.37}            \\ \bottomrule
\end{tabular}
\caption{Automatic evaluations on detoxified generations on the microagressions.com Tumblr dataset for \methodname, ParaGeDi and CondBERT. \methodname achieves the lowest toxicity and best fluency, and the second-best meaning preservation metrics. CondBERT achieves the highest BERTScore and BLEU4. }
\label{tab:1}
\end{table}

% \begin{table*}[t]
% \footnotesize
% \centering
% \begin{tabular}{lllllllll}
% \toprule
%           & \multicolumn{4}{c}{Validation}         & \multicolumn{4}{c}{Test}               \\
%           \cmidrule(lr){2-5}  \cmidrule(lr){6-9}
%           & Toxicity & BERTScore & BLEU4 & Fluency & Toxicity  & BERTScore& BLEU4 & Fluency \\ \midrule
% Original & 0.286  & --	 & 	-- &         80.54        &       &         \\
% CondBERT &   \underline{0.161}	& \textbf{0.966} &	\textbf{0.800} &	\underline{114.27}               &           &         \\
% ParaGeDi  &     0.162	& 0.931 &	0.499&	140.86               &           &         \\
% MaRCo     &      \textbf{0.145} & \underline{0.958} &	\underline{0.768} &	\textbf{61.37}              &           &       \\ \bottomrule
% \end{tabular}
% \caption{Automatic evaluations on detoxified generations on the microagressions.com Tumblr dataset for \methodname, ParaGeDi and CondBERT. \methodname achieves the lowest toxicity and best fluency, and the second-best meaning preservation metrics. CondBERT achieves the highest BERTScore and BLEU4. }
% \label{tab:1}
% \end{table*}

% \begin{figure}
%     \centering
% \includegraphics[width=0.5\textwidth]{images/microagressions_humaneval_marco_paragedi.png}
%     \includegraphics[width=0.5\textwidth]{images/microagressions_humaneval_condbert_marco.png}
%     \caption{Human evaluations on detoxified generations on the microagressions.com Tumblr dataset for \methodname vs ParaGeDi and for \methodname vs CondBERT. \methodname has less-toxic and more fluent generations, while both CondBERT and ParaGeDi has more meaning preservation.}
%     \label{fig:micro_para_marco}
% \end{figure}

==> tables/sbf.tex <==
\begin{table}[t]
\footnotesize
\centering
\begin{tabular}{lllll}
\toprule
          & \multicolumn{4}{c}{Validation}              \\
          \cmidrule(lr){2-5}  \
          & Toxicity & BERTScore& BLEU4 & Fluency \\ \midrule
Original &   0.351	& --	 & 	-- &268.53         \\
CondBERT &   \underline{0.202}	&	\textbf{0.961} & \textbf{0.770}	& \underline{98.11}                \\
ParaGeDi  &     0.186 &		0.921 &	0.462 &	131.76        \\
MaRCo     &     \textbf{0.176}	&	\underline{0.947}	& \underline{0.732} &	\textbf{71.80}     \\ \bottomrule
\end{tabular}
\caption{Automatic evaluations on detoxified generations on SBF for \methodname, ParaGeDi and CondBERT. \methodname achieves the lowest toxicity and best fluency, and the second-best meaning preservation metrics. CondBERT achieves the highest BERTScore and BLEU4. }
\label{tab:2}
\end{table}

% \begin{table*}[t]
% \footnotesize
% \centering
% \begin{tabular}{lllllllll}
% \toprule
%           & \multicolumn{4}{c}{Validation}         & \multicolumn{4}{c}{Test}               \\
%           \cmidrule(lr){2-5}  \cmidrule(lr){6-9}
%           & Toxicity & BERTScore& BLEU4 & Fluency & Toxicity& BERTScore & BLEU4  & Fluency \\ \midrule
% Original &   0.351	& --	 & 	-- &268.53                  &       &         \\
% CondBERT &   \underline{0.202}	&	\textbf{0.961} & \textbf{0.770}	& \underline{98.11}              &           &         \\
% ParaGeDi  &     0.186 &		0.921 &	0.462 &	131.76   &           &        \\
% MaRCo     &     \textbf{0.176}	&	\underline{0.947}	& \underline{0.732} &	\textbf{71.80}         &           &       \\ \bottomrule
% \end{tabular}
% \caption{Automatic evaluations on detoxified generations on SBF for \methodname, ParaGeDi and CondBERT. \methodname achieves the lowest toxicity and best fluency, and the second-best meaning preservation metrics. CondBERT achieves the highest BERTScore and BLEU4. }
% \label{tab:2}
% \end{table*}
